IKA: Independent Kernel Approximator

This paper describes a new method for low rank kernel approximation called IKA. The main advantage of IKA is that it produces a function $\psi(x)$ defined as a linear combination of arbitrarily chosen functions. In contrast the approximation produced by Nystr\"om method is a linear combination of kernel evaluations. The proposed method consistently outperformed Nystr\"om method in a comparison on the STL-10 dataset. Numerical results are reproducible using the source code available at https://gitlab.com/matteo-ronchetti/IKA

==> cmds/commands.tex <==
\newcommand{\notationref}{see notation on page \pageref{notation} }

\newcommand{\theoremref}[1]{\ref{#1} on page \pageref{#1}}


\newcommand\opn{\mathrel{\ooalign{$\subseteq$\cr
  \hidewidth\raise.225ex\hbox{$\circ\mkern.5mu$}\cr}}}

\newcommand{\limeps}{\lim_{\epsilon \to 0}}

\newcommand{\system}[1]{\left\{\begin{array}{ll} #1 \end{array}\right.}




\newcommand{\colmatrix}[2]{
\left( \begin{array}{c|c|c|c}
    &   & &\\ 
#1_1 & #1_2 & ... & #1_#2 \\
    &  &  &\\
 \end{array} \right)
}
\newcommand{\colmatrixp}[3]{
\left( \begin{array}{c|c|c|c}
    &   & &\\ 
#1 & #2 & ... & #3 \\
    &  &  &\\
 \end{array} \right)
}


\newcommand{\Def}[2]{
\vspace{5mm}
\textbf{#1} 
\reversemarginpar \marginnote{\textcolor{defgray}{\textsf{\textbf{Def}}}} \\
#2
\vspace{5mm}
}
